Convolution of Scale Invariant Continuous Ranked Probability Scores for Testing Experts' Statistical Accuracy

Computable solutions for expectations of Continuous Ranked Probability Scores are presented. After deriving a scale invariant version of these scores, a closed form for the convolutions of scores is presented. This closed form enables the testing experts' statistical accuracy. Results are compared with tests using a familiar Chi-square goodness of fit test using a recent data set of 6,761 expert probabilistic forecasts for which true values are known.

==> refs.tex <==


@article{ray2020ensemble,
  title={Ensemble forecasts of coronavirus disease 2019 (covid-19) in the us},
  author={Ray, Evan L and Wattanachit, Nutcha and Niemi, Jarad and Kanji, Abdul Hannan and House, Katie and Cramer, Estee Y and Bracher, Johannes and Zheng, Andrew and Yamana, Teresa K and Xiong, Xinyue and others},
  journal={MedRXiv},
  year={2020},
  publisher={Cold Spring Harbor Laboratory Press}
}
@article{Candille&Talagrand2005,
title= {Evaluation of probabilistic prediction systems for a scalar variable},
      author = {Candille, G. and Talagrand, O.},
      journal = {Q.J.R.Meteorool. Soc},
      year = {2005},
      publisher = {Royal Meteorological Society},
      volume = {131},
      pages= {2131 -- 2150},
      doi = 
}

@article{Hersbach2000,
  title={Decomposition of the Continuous Ranked Probability Score for Ensemble Prediction Systems},
  author={ Hersbach, H.},
  journal={Weather and Forecasting},
  volume={15},
  pages={559--570},
  year={2000},
  }

@article{Aitchison&Dunsmore68,
  title={Linear-loss interval estimation of location and scale parameters},
  author={ Aitchison,J. and Dunsmore, I.R. },
  journal={Biometrica},
  volume={55},
  number={1},
  pages={141--148},
  year={1968},
  }
@article{cramer2022evaluation,
  title={Evaluation of individual and ensemble probabilistic forecasts of COVID-19 mortality in the United States},
  author={Cramer, Estee Y and Ray, Evan L and Lopez, Velma K and Bracher, Johannes and Brennen, Andrea and Castro Rivadeneira, Alvaro J and Gerding, Aaron and Gneiting, Tilmann and House, Katie H and Huang, Yuxin and others},
  journal={Proceedings of the National Academy of Sciences},
  volume={119},
  number={15},
  pages={e2113561119},
  year={2022},
  publisher={National Acad Sciences}
}

@article{reich2019accuracy,
  title={Accuracy of real-time multi-model ensemble forecasts for seasonal influenza in the US},
  author={Reich, Nicholas G and McGowan, Craig J and Yamana, Teresa K and Tushar, Abhinav and Ray, Evan L and Osthus, Dave and Kandula, Sasikiran and Brooks, Logan C and Crawford-Crudell, Willow and Gibson, Graham Casey and others},
  journal={PLoS computational biology},
  volume={15},
  number={11},
  pages={e1007486},
  year={2019},
  publisher={Public Library of Science San Francisco, CA USA}
}

@article{cramer2021evaluation,
  title={Evaluation of individual and ensemble probabilistic forecasts of COVID-19 mortality in the US},
  author={Cramer, Estee Y and Ray, Evan L and Lopez, Velma K and Bracher, Johannes and Brennen, Andrea and Rivadeneira, Alvaro J Castro and Gerding, Aaron and Gneiting, Tilmann and House, Katie H and Huang, Yuxin and others},
  journal={Medrxiv},
  year={2021},
  publisher={Cold Spring Harbor Laboratory Press}
}

@article{bracher2021evaluating,
  title={Evaluating epidemic forecasts in an interval format},
  author={Bracher, Johannes and Ray, Evan L and Gneiting, Tilmann and Reich, Nicholas G},
  journal={PLoS computational biology},
  volume={17},
  number={2},
  pages={e1008618},
  year={2021},
  publisher={Public Library of Science San Francisco, CA USA}
}
@article{Brown74,
author={Brown, Thomas A.},
title={Admissible Scoring Systems for Continuous Distributions},
year={1974},
journal={RAND Corporation}
}
@article{Matheson76,
title = {Scoring Rules for Continuous Probability Distributions},
author = {Matheson, James E. and Winkler, Robert L.},
year = {1976},
journal = {Management Science},
volume = {22},
number = {10},
pages = {1087-1096},
url = {https://EconPapers.repec.org/RePEc:inm:ormnsc:v:22:y:1976:i:10:p:1087-1096}
}
@inproceedings{Talarand76,
  author = {O. Talagrand and R. Vautard and B Strauss},
  title = {Evaluation of probabilistic prediction systems},
  year = {1997},
  journal = {Workshop on Predictability, 20-22 October 1997},
  pages = {1-26},
  month = {1997},
  publisher = {ECMWF},
  address = {Shinfield Park, Reading},
  language = {eng},
}

@article{bamber2016commentary,
  title={A commentary on “how to interpret expert judgment assessments of twenty-first century sea-level rise” by Hylke de Vries and Roderik SW van de Wal},
  author={Bamber, Jonathan L and Aspinall, Willy P and Cooke, Roger M},
  journal={Climatic Change},
  volume={137},
  number={3},
  pages={321--328},
  year={2016},
  publisher={Springer}
}


@article{colson2017cross,
  title={Cross validation for the classical model of structured expert judgment},
  author={Colson, Abigail R and Cooke, Roger M},
  journal={Reliability Engineering \& System Safety},
  volume={163},
  pages={109--120},
  year={2017},
  publisher={Elsevier}
}

@article{cooke2021expert,
  title={Expert forecasting with and without uncertainty quantification and weighting: What do the data say?},
  author={Cooke, Roger M and Marti, Deniz and Mazzuchi, Thomas},
  journal={International Journal of Forecasting},
  volume={37},
  number={1},
  pages={378--387},
  year={2021},
  publisher={Elsevier}
}

@article{cooke2018probabilistic,
  title={Probabilistic reasoning about measurements of equilibrium climate sensitivity: combining disparate lines of evidence},
  author={Cooke, Roger M and Wielicki, Bruce},
  journal={Climatic change},
  volume={151},
  number={3},
  pages={541--554},
  year={2018},
  publisher={Springer}
}

@book{cooke1991experts,
  title={Experts in uncertainty: opinion and subjective probability in science},
  author={Cooke, Roger M},
  year={1991},
  publisher={Oxford University Press on Demand}
}

@article{cooke2014validating,
  title={Validating expert judgment with the classical model},
  author={Cooke, Roger M},
  journal={Experts and consensus in social science},
  pages={191--212},
  year={2014},
  publisher={Springer}
}

@incollection{cooke2018vldcm,
title={Validation in the Classical Model},
author={Cooke, Roger M},
booktitle={Elicitation; The Science and Art of Structuring Judgement},
editors={Luis C. Dias, Alec Morton, John Quigley},
pages={37--59},
year={2018},
publisher={Springer}
}

@article{cramer2022evaluation,
  title={Evaluation of individual and ensemble probabilistic forecasts of COVID-19 mortality in the United States},
  author={Cramer, Estee Y and Ray, Evan L and Lopez, Velma K and Bracher, Johannes and Brennen, Andrea and Castro Rivadeneira, Alvaro J and Gerding, Aaron and Gneiting, Tilmann and House, Katie H and Huang, Yuxin and others},
  journal={Proceedings of the National Academy of Sciences},
  volume={119},
  number={15},
  pages={e2113561119},
  year={2022},
  publisher={National Acad Sciences}
}

@inproceedings{de1937prevision,
  title={La pr{\'e}vision: ses lois logiques, ses sources subjectives},
  author={De Finetti, Bruno},
  booktitle={Annales de l'institut Henri Poincar{\'e}},
  volume={7},
  number={1},
  pages={1--68},
  year={1937}
}

@article{degroot1983comparison,
  title={The comparison and evaluation of forecasters},
  author={DeGroot, Morris H and Fienberg, Stephen E},
  journal={Journal of the Royal Statistical Society: Series D (The Statistician)},
  volume={32},
  number={1-2},
  pages={12--22},
  year={1983},
  publisher={Wiley Online Library}
}

@article{gneiting2007strictly,
  title={Strictly proper scoring rules, prediction, and estimation},
  author={Gneiting, Tilmann and Raftery, Adrian E},
  journal={Journal of the American statistical Association},
  volume={102},
  number={477},
  pages={359--378},
  year={2007},
  publisher={Taylor \& Francis}
}

@article{gneiting2007jrss,
  title={Probabilistic forecasts, calibration and sharpness},
  author={Gneiting, Tilmann and Balabdaoui, Fadoua  and Raftery, Adrian E},
  journal={J. R. Statist. Soc. B  Part 2},
  volume={69},
   pages={243--368},
  year={2007},
  publisher={Royal Statistical Society}
}



@article{lichtendahl2013better,
  title={Is it better to average probabilities or quantiles?},
  author={Lichtendahl Jr, Kenneth C and Grushka-Cockayne, Yael and Winkler, Robert L},
  journal={Management Science},
  volume={59},
  number={7},
  pages={1594--1611},
  year={2013},
  publisher={INFORMS}
}

@article{murphy1977value,
  title={The value of climatological, categorical and probabilistic forecasts in the cost-loss ratio situation},
  author={Murphy, Allan H},
  journal={Monthly Weather Review},
  volume={105},
  number={7},
  pages={803--816},
  year={1977}
}

@article{rougier2013second,
  title={Second-order exchangeability analysis for multimodel ensembles},
  author={Rougier, Jonathan and Goldstein, Michael and House, Leanna},
  journal={Journal of the American Statistical Association},
  volume={108},
  number={503},
  pages={852--863},
  year={2013},
  publisher={Taylor \& Francis}
}

@article{shuford1966admissible,
  title={Admissible probability measurement procedures},
  author={Shuford, Emir H and Albert, Arthur and Edward Massengill, H},
  journal={Psychometrika},
  volume={31},
  number={2},
  pages={125--145},
  year={1966},
  publisher={Springer}
}


@article{weissman2017sum,
  title={Sum of squares of uniform random variables},
  author={Weissman, Ishay},
  journal={Statistics \& Probability Letters},
  volume={129},
  pages={147--154},
  year={2017},
  publisher={Elsevier}
}

@article{forrester2018comment,
  title={Comment on “Sum of squares of uniform random variables” by I. Weissman},
  author={Forrester, Peter J},
  journal={Statistics \& Probability Letters},
  volume={142},
  pages={118--122},
  year={2018},
  publisher={Elsevier}
}

@article{xu1996volume,
  title={The volume of the intersection of a cube and a ball in n-space},
  author={Xu, Liqun},
  journal={SIAM Review},
  volume={38},
  number={4},
  pages={669--669},
  year={1996},
  publisher={SIAM}
}

@article{RousseauRuehr1997,
  title={ Problems and solutions. subsection: The volume of the intersection of a cube and a ball in N-space. two solutions by Bernd Tibken and Denis Constales},
  author={Rousseau, C.C. and Ruehr, O.G.},
  journal={SIAM Review},
  volume={39},
  number={4},
  pages={779–786},
  year={1997},
  publisher={SIAM}
}

@article{savage1971elicitation,
  title={Elicitation of personal probabilities and expectations},
  author={Savage, Leonard J},
  journal={Journal of the American Statistical Association},
  volume={66},
  number={336},
  pages={783--801},
  year={1971},
  publisher={Taylor \& Francis}
}

@article{morley2018measures,
  title={Measures of model performance based on the log accuracy ratio},
  author={Morley, Steven Karl and Brito, Thiago Vasconcelos and Welling, Daniel T},
  journal={Space Weather},
  volume={16},
  number={1},
  pages={69--88},
  year={2018},
  publisher={Wiley Online Library}
}

@article{flandoli2011comparison,
  title={Comparison of a new expert elicitation model with the Classical Model, equal weights and single experts, using a cross-validation technique},
  author={Flandoli, Franco and Giorgi, Enrico and Aspinall, William P and Neri, Augusto},
  journal={Reliability Engineering \& System Safety},
  volume={96},
  number={10},
  pages={1292--1310},
  year={2011},
  publisher={Elsevier}
}

@article{borchers2022package,
  title={Package ‘pracma’},
  author={Borchers, Hans W and Borchers, Maintainer Hans W},
  journal={accessed on},
  volume={4},
  year={2022}
}

@book{billingsley2013convergence,
  title={Convergence of probability measures},
  author={Billingsley, Patrick},
  year={2013},
  publisher={John Wiley \& Sons}
}

@article{hanea2021depth,
  title={An in-depth perspective on the classical model},
  author={Hanea, Anca M and Nane, Gabriela F},
  journal={Expert Judgement in Risk and Decision Analysis},
  pages={225--256},
  year={2021},
  publisher={Springer}
}
